Learning Two-input Linear and Nonlinear Analog Functions with a Simple Chemical System

The current biochemical information processing systems behave in a predetermined manner because all features are defined during the design phase. To make such unconventional computing systems reusable and programmable for biomedical applications, adaptation, learning, and self-modification based on external stimuli would be highly desirable. However, so far, it has been too challenging to implement these in wet chemistries. In this paper we extend the chemical perceptron, a model previously proposed by the authors, to function as an analog instead of a binary system. The new analog asymmetric signal perceptron learns through feedback and supports Michaelis-Menten kinetics. The results show that our perceptron is able to learn linear and nonlinear (quadratic) functions of two inputs. To the best of our knowledge, it is the first simulated chemical system capable of doing so. The small number of species and reactions and their simplicity allows for a mapping to an actual wet implementation using DNA-strand displacement or deoxyribozymes. Our results are an important step toward actual biochemical systems that can learn and adapt.

==> x_abstract_chemical_learning_system.tex <==
\section{Abstract Chemical Learning System and Its Implications}
\label{sec:abstract-chemical-learning-system}
%-----------------------------------------------------------

In an abstract chemical learning system, we can categorize species
into four groups: input, output, functional, and feedback. The weight
species of our chemical perceptrons are specific examples of
functional species, and the desired output and the penalty signal
showcase feedback species. The concentration of the functional species constitutes the behaviour of
the system, and therefore it must be
preserved during regular execution, so multiple inputs can be fed into
the system sequentially. The most natural choice to achieve that is to
make the functional species the catalysts that drive the
input-to-output reactions, as we did. The learning module prescribes
how the system should behave, and it adjusts the concentration of the functional species if needed.

%Elaborate how learning is done
%How to incorporate computing usefulness to the model of life.

The application of the learning module goes beyond learning: from a
computer science perspective, the functional species guide the
chemical execution and therefore represent the low-level (chemical)
code. The specification of the learning module in terms of input and
desired output pairs represents the high-level functional program. In the
process of learning, a program compiles to the chemical code of the
functional species concentrations, hence, the learning module
introduces the compilation layer, bridging computer science and
chemistry, allowing users without a background in chemistry to
effectively program this chemical interface. Note that, as opposed to
the ordinary procedural programming, the functional programming does
not say \textit{how} we want to achieve our goal in a step-by-step
fashion but specifies instead \textit{what} behaviour we want our
system to imitate.

Another interesting dimension of chemical learning comes from the
\textit{Systems and Relational Biology} \cite{bertalanffy1968,kitano2002}. In living organisms the
metabolic transformation of substrates $A$ to products $B$ is
catalysed by functional species (enzymes) $f$\cite{piedrafita2010}. 
Rosen\cite{rosen1991} distinguishes between
the material causation $A \rightarrow B$ and the efficient causation
$f \Longrightarrow (A \rightarrow B)$ and asserts that life must be
open to material, but closed to efficient causation. The problem here
is that the metabolic catalysts undergo decay due to dilution and
their finite stability, hence an organism must continuously recreate
them by an inner repair (replacement) mechanism, so they must be the
product of metabolism as well. Rosen's $(M,R)$ system (standing for
the metabolic-repair or metabolic-replacement system) generalizes this
idea and explicitly assumes the material link between the product of
metabolism $B$ and the catalysts $f$ controlled by the replacement
system $\Phi$. The replacement system is, however, physical, and
therefore subject to decay. To avoid infinite regress, Rosen
postulated the replication of $\Phi$ from the catalysts $f$ with
efficient causation of metabolites $B$ obtaining the organization
invariance of the system.

If we draw a diagram of a chemical learning system next to Rosen's
diagram of life, as in
Figure\ref{fig:rosen_and_learning_system_diagrams}, we can see
striking parallels. Note that to be consistent with the $(M,R)$
formalism we renamed the species accordingly. The transformation of
the input to the output species in a chemical learning system is
essentially metabolism, although our interpretation of the output
(product) has a \textit{meaning} and is available for external
measurement. Furthermore, the (re)creation of the functional species
$f$ in our model, called adaptation, is driven by the learning module
$\Phi_L$, as opposed to the term regulatory replacement operated by
$\Phi$. The main structural difference and also a simplification we
adopted is that our functional species do not decay,
so we did not have to deal with explicit replacement. The learning
module prescribes the expected behaviour, hence
if the weights decayed and their concentrations diverted outside the
desired region, and therefore produced incorrect output, the learning
module would detect that and recover or stabilize the
concentrations. Thus, if the learning module were invoked internally on a regular basis rather than an external
cause, it would form its function factory, and consequently Rosen's
replacement mechanism. This gives an interesting relation between
individual learning, wherein the learning module is driven by an
environment or a teacher, and population learning (evolution), wherein
individuals share the hard-coded internal function factory with
input-output pairs encoded in the genome. Although a function factory
is in place and continually repairs an underlying function species, we
still have to deal with the problem of its own degradation. Besides
that, we can perhaps keep one instance of the learning module to
maintain the function and one for individual learning (adaptation of
function).

% how learning fits to the definition of life
% concentration stabilization part

Here, we showed that the learning is not just about adaptation to the
feedback from the environment, but it encompasses the more general
area of self-stabilization. Whether we should call this process
learning, programming, regulation, replacement, or repair is
ultimately strictly based on the purpose of what we consider a general
function factory.

% We have explored also the way to reconstruct functional species after each processing but this approach is rather cumbersome (the weight-loop perceptron model). 

\begin{figure}[ht!]
  \centering
  \subfigure[] {
     \includegraphics[width=.4\textwidth]{Rosen_diagram}
     \label{fig:Rosen_diagram}
  }
  \subfigure[] {
     \includegraphics[width=.4\textwidth]{learning_system_diagram}
     \label{fig:learning_system_diagram}
  }
  \caption{(a) Rosen's diagram showing organization invariance of
    life. The system is continually repaired and replicated as a product
    of its own metabolism. Solid arrows are material causations,
    whereas dashed arrows are efficient causations; (b) High-level
    diagram of an abstract chemical learning system. The concentration
    of functional species is adapted by the learning module
    implemented internally and operated externally by a trainer.}
  \label{fig:rosen_and_learning_system_diagrams}
\end{figure}

